Generalised Mutual Information: a Framework for Discriminative Clustering

In the last decade, recent successes in deep clustering majorly involved the Mutual Information (MI) as an unsupervised objective for training neural networks with increasing regularisations. While the quality of the regularisations have been largely discussed for improvements, little attention has been dedicated to the relevance of MI as a clustering objective. In this paper, we first highlight how the maximisation of MI does not lead to satisfying clusters. We identified the Kullback-Leibler divergence as the main reason of this behaviour. Hence, we generalise the mutual information by changing its core distance, introducing the Generalised Mutual Information (GEMINI): a set of metrics for unsupervised neural network training. Unlike MI, some GEMINIs do not require regularisations when training as they are geometry-aware thanks to distances or kernels in the data space. Finally, we highlight that GEMINIs can automatically select a relevant number of clusters, a property that has been little studied in deep discriminative clustering context where the number of clusters is a priori unknown.

==> figs_tex/enron/fig_cmatrix_gemini_deep_lpm.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/enron_cmatrix_deep_lpm_gemini.pdf}
    \caption{Confusion matrix between both clustering assignments according to the Deep LPM model and the GEMINI model. The ARI between both clustering is 54\%.}
    \label{fig:confusion_matrix_lpm_gemini}
\end{figure}

==> figs_tex/enron/fig_employee_status_distribution.tex <==
\begin{figure}[!ht]
	\centering
	\subfloat[GEMINI]{
	\includegraphics[width=0.48\linewidth]{figs/enron_cmatrix_status_gemini.pdf}\label{sfig:status_distribution_gemini}}\hfil
	\subfloat[Deep LPM]{\includegraphics[width=0.48\linewidth]{figs/enron_cmatrix_status_dlpm.pdf}\label{sfig:status_distribution_dlpm}}
	\caption{Distribution of status of employees per cluster. The GEMINI clusters are reordered to match at best the distribution of the Deep LPM clusters, following the confusion matrix from Figure~\ref{fig:confusion_matrix_lpm_gemini}.}
	\label{fig:status_distribution}
\end{figure}

==> figs_tex/enron/fig_gemini_training_curves.tex <==
\begin{figure*}[!ht]
    \centering
    \subfloat[GEMINI training curve]{\includegraphics[width=0.3\linewidth]{figs/enron_gemini_loss_history.pdf}}\hfil
    \subfloat[Number of samples changing assignment per epoch]{\includegraphics[width=0.3\linewidth]{figs/enron_stability_history.pdf}}\hfil
    \subfloat[Number of clusters]{\includegraphics[width=0.3\linewidth]{figs/enron_gemini_clusters_history.pdf}}
    \caption{Training curves for the best GEMINI model on the Enron email interaction dataset. The first 6000 epochs are done with the OvA Wasserstein and the 2000 remaining after the red lines are done with the OvO Wasserstein.}
    \label{fig:enron_training_history}
\end{figure*}
